BLINC: Blind Calibration For Training-Free Speech Enhancement Adaptation

Speech enhancement (SE) models degrade under domain shifts and have to adapt to unseen target domains during deployment. Most existing test-time adaptation (TTA) methods for SE do so by adapting a subset of the model weights using a self-supervised loss, which requires backpropagation at test-time and permanently alters the model. We instead recalibrate the prediction itself and propose BLINC, a training-free TTA method that remaps the predicted time-frequency mask onto a bimodal target distribution by histogram matching. At test-time, the target distribution is parameterized from blind features of the noisy recording, so neither a reference distribution from a classical algorithm nor online metric optimization is involved. BLINC improves the overall quality of both evaluated SE models on almost every target condition and matches or exceeds the loss-based TTA baselines at minimal overhead.

==> fig/data/dist_order.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
            xtick={1},
			xticklabel={\empty},
			ymin=0.0, ymax=3000,
			xmin=-0.2, xmax=1.2,
			width=10em, height=8em,
		]

        \addplot[mittelgrau, fill=mittelgrau!50, line width=1pt]
		coordinates {
				(-0.001, 0)
				(0, 800)
                (1, 800)
                (1.001, 0)
			};

	\end{axis}
\end{tikzpicture}


==> fig/data/dist_pred.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
            xtick={1},
			xticklabel={\empty},
			ymin=0.0, ymax=3000,
			xmin=-0.2, xmax=1.2,
			width=10em, height=8em,
		]

		\addplot[mittelblau, fill=mittelblau!50, fill opacity=0.7, line width=1pt]
		table [x=x, y=y]
			{fig/data/pred.txt};
	\end{axis}
\end{tikzpicture}


==> fig/data/dist_pred_small.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
            xtick=\empty,
			xticklabel={\empty},
			ymin=0.0, ymax=3000,
			xmin=-0.2, xmax=1.2,
			width=7em, height=7em,
		]

		\addplot[mittelblau, fill=mittelblau!50, fill opacity=0.7, line width=1pt]
		table [x=x, y=y]
			{fig/data/pred_small.txt};
	\end{axis}
\end{tikzpicture}


==> fig/data/dist_regress.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
            xtick={1},
			xticklabel={\empty},
			ymin=0.0, ymax=3000,
			xmin=-0.2, xmax=1.2,
			width=10em, height=8em,
		]

		\addplot[orange, fill=orange!50, fill opacity=0.7, line width=1pt]
		table [x=x, y=y]
			{fig/data/regress.txt};

	\end{axis}
\end{tikzpicture}


==> fig/data/dist_regress_small.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
            xtick=\empty,
			xticklabel={\empty},
			ymin=0.0, ymax=3000,
			xmin=-0.2, xmax=1.2,
			width=7em, height=7em,
		]

		\addplot[orange, fill=orange!50, fill opacity=0.7, line width=1pt]
		table [x=x, y=y]
			{fig/data/regress_small.txt};

	\end{axis}
\end{tikzpicture}


==> fig/misc/mini_blinc.tex <==
\begin{tikzpicture}
	\tikzstyle{model} = [rectangle, draw=black, inner sep=1em, align=center]
	\tikzstyle{helper} = [inner sep=3pt]
	\tikzstyle{stft} = [inner sep=0pt]
	\tikzstyle{mult} = [inner sep=0.8pt, circle, align=center, text centered, label={[font=\large]center:\(\odot\)}]
	\tikzstyle{bound} = [inner sep=5pt, draw, dashed, rounded corners=\corner]
	\tikzstyle{bound_l} = [inner sep=4pt, draw, rounded corners=\scorner]
	\tikzstyle{hist} = [inner sep=0pt]

	\node (hist_1) [hist] {\resizebox{3.5em}{!}{\input{fig/data/dist_pred_small.tex}}};
	\node (hist_2) [hist, right=1.5em of hist_1] {\resizebox{3.5em}{!}{\input{fig/data/dist_regress_small.tex}}};
	\draw [arrow] (hist_1) -- (hist_2);


\end{tikzpicture}


==> fig/misc/reg_a.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis lines=left,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
            ymin=0.0, ymax=1.0,
			width=3cm, height=3cm,
		]

		\addplot [
			domain=0.0:1.0,
			samples=5,
			line width=2pt,
			color=mauve,
		]
		{-0.1 * x + 0.5};

	\end{axis}
\end{tikzpicture}


==> fig/misc/reg_d.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis lines=left,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
            ymin=0.0, ymax=1.0,
			width=3cm, height=3cm,
		]

		\addplot [
			domain=0.0:1.0,
			samples=5,
			line width=2pt,
			color=lila,
		]
		{-0.5 * x + 0.75};

	\end{axis}
\end{tikzpicture}


==> fig/misc/reg_s.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis lines=left,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
			width=3cm, height=3cm,
			ymin=0.0, ymax=1.0,
		]

		\addplot [
			domain=0.0:1.0,
			samples=5,
			line width=2pt,
			color=pink,
		]
		{0.5 * x + 0.1};

	\end{axis}
\end{tikzpicture}


==> fig/quantile_schem.tex <==
\begin{tikzpicture}
	\begin{axis}[
            axis lines=left,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
            ymin=-0.2, ymax=1.1,
			width=4cm, height=3.5cm,
			clip mode=individual,
		]

		\addplot [
			domain=0.0:1.0,
			samples=50,
			color=lavendel,
            line width=2pt,
		]
		{max(min(1.01*(1/(1+exp(-8.5*(x-0.5)))) - 0.01, 1.0), 0.0)};

        \draw[arrow, pink] (0.5, 0.5) -- (0.3, 0.5);
        \draw[arrow, pink] (0.5, 0.5) -- (0.7, 0.5);

        \draw[arrow, lila] (0.1, 0.0226) -- (0.1, -0.15);
        \draw[arrow, lila] (0.1, 0.0226) -- (0.1, 0.1726);

		\draw[arrow, mauve] (0.7, 0.844) -- (0.8, 0.844);
		\draw[arrow, mauve] (0.7, 0.844) -- (0.6, 0.844);
		\draw[arrow, mauve] (0.3, 0.146) -- (0.2, 0.146);
		\draw[arrow, mauve] (0.3, 0.146) -- (0.4, 0.146);

	\end{axis}
\end{tikzpicture}

